"Private Prediction Strikes Back!'' Private Kernelized Nearest Neighbors with Individual Renyi Filter

Most existing approaches of differentially private (DP) machine learning focus on private training. Despite its many advantages, private training lacks the flexibility in adapting to incremental changes to the training dataset such as deletion requests from exercising GDPR's right to be forgotten. We revisit a long-forgotten alternative, known as private prediction, and propose a new algorithm named Individual Kernelized Nearest Neighbor (Ind-KNN). Ind-KNN is easily updatable over dataset changes and it allows precise control of the R\'{e}nyi DP at an individual user level -- a user's privacy loss is measured by the exact amount of her contribution to predictions; and a user is removed if her prescribed privacy budget runs out. Our results show that Ind-KNN consistently improves the accuracy over existing private prediction methods for a wide range of $\epsilon$ on four vision and language tasks. We also illustrate several cases under which Ind-KNN is preferable over private training with NoisySGD.

==> 04_motivation.tex <==
\section{Motivation}

%In this section, we revisit a few challenges faced in the practical deployment of private machine learning models, which motivates our work.


%One of the major challenges is the prevalence of data poisoning attacks. In these attacks, an adversary manipulates the training data in order to mislead the learned model. Despite the design of DP models to limit the influence of individual data points, these models can still be vulnerable to data poisoning attacks (see \citet{ma2019data}). Defending against data poisoning attacks while ensuring privacy is a complex problem that requires the development of robust methods for detecting and mitigating the impact of malicious data points on the DP model.

%Another important aspect to consider is that there are privacy regulations beyond membership privacy (offered by DP) that must be taken into account in practice.  As we discussed in the introduction,  machine unlearning  gives individuals the right to delete their data and requires machine learning models to ``unlearn'' what they have learned from it. However, erasing the impact of deleted data from DP models can be challenging due to the randomized nature of the training process. 



Private training using NoisySGD~\citep{abadi} has become the standard method for achieving differential privacy in ML. However, one drawback of private training its resource intensiveness, especially when combined with recent techniques that improve its privacy-utility trade-off~\citep{li2021large, yu2021differentially, de2022unlocking}. In practice, training is rarely a one-time process since models often need to be updated to remove corrupted data~\citep{chen2017targeted, jagielski2018manipulating} or to satisfy the so-called \emph{right to be forgotten} via machine unlearning~\citep{ginart2019making, guo2019certified, bourtoule2021machine}.
 Periodic retraining of models can help mitigate the above issues, but it comes at a significant computational and privacy cost.
 
 The following example empirically quantifies the computational and privacy cost of retraining on CIFAR-10.
 Consider a private prediction task where a DP model is trained on a private dataset to respond to a stream of queries. We assume that a retraining request will be received every time the model has answered $Q$ queries. To simplify the analysis, we will use the training set of CIFAR-10 as the private set and assume that each retraining is performed on the same dataset.  We use the  Linear NoisySGD~\citep{tramer2020differentially} model for illustration, which trains a DP linear model over the feature representation of each input. We train Linear NoisySGD for $10$ epochs on the private set. % The per-query computational cost is calculated by summing the total time spent on retraining and answering a total of $T=10000$ queries, and then dividing the result by $T$. This provides an estimate of the average time required to answer a single query.
 
 For privacy cost, note that privacy loss composes over multiple training rounds. At a given retraining frequency $Q$, we calculate privacy loss over $\frac{T}{Q}$ training rounds. The privacy  hyper-parameter (e.g., noise multiplier, batch size) is chosen such that the accuracy of labeled queries is $82\%$.
  As shown in Figure~\ref{fig: speed_eps},  computational and privacy costs increase rapidly as the frequency increases.
  % in the exp, we empirically compare 

\begin{figure}[!htb]
\centering
\includegraphics[width=0.9\linewidth]{ind_knn/img/speed_eps.pdf}
\caption{Computational cost and privacy loss of answering $T=10000$ queries of NoisySGD on CIFAR-10 with periodic retraining. The x-axis indicates the retraining frequency, i.e.,  the number of queries $Q$ received before retraining the model, the smaller $Q$ resulting in a higher frequency.  The left y-axis plots the estimated computational cost, which is calculated by summing the total time spent on retraining and dividing  by $T$.
The right y-axis plots the total privacy loss of answering T queries, which increases rapidly as the retraining frequency increases. }
\label{fig: speed_eps}
\end{figure}

==> 07_related.tex <==
\section{Related Works}
Private kNN~\citep{zhu2020private} is a private prediction mechanism that addresses the shortcomings of private training by performing nearest neighbor search in the embedding space of a pre-trained network. It reduces the training cost to maintaining the training set embeddings and allows on-the-fly addition and removal of training samples. However, the privacy cost of Private kNN accumulates quickly under repeated queries, making it uncompetitive to private training.

DP-SGD~\citep{abadi2016deep} is the predominant method for applying differential privacy to machine learning and relies on private training. It requires per-sample gradient computation, which is much more computation- and memory-intensive than standard training. Recent advancements, such as large batch training~\citep{li2021large, yu2021differentially} and multiple augmentations~\citep{de2022unlocking}, have pushed the state-of-the-art in private training but have increased the computation cost even further.

The R\'{e}nyi filter~\citep{feldman2021individual} is used in this work to account for the privacy cost of each sample individually. This allows each training sample to participate in the query response until its own privacy budget is exhausted, reducing the privacy cost for common queries.


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
